Tight Lower Bounds for Directed Cut Sparsification and Distributed Min-Cut

In this paper, we consider two fundamental cut approximation problems on large graphs. We prove new lower bounds for both problems that are optimal up to logarithmic factors. The first problem is to approximate cuts in balanced directed graphs. In this problem, the goal is to build a data structure that $(1 \pm \epsilon)$-approximates cut values in graphs with $n$ vertices. For arbitrary directed graphs, such a data structure requires $\Omega(n^2)$ bits even for constant $\epsilon$. To circumvent this, recent works study $\beta$-balanced graphs, meaning that for every directed cut, the total weight of edges in one direction is at most $\beta$ times that in the other direction. We consider two models: the {\em for-each} model, where the goal is to approximate each cut with constant probability, and the {\em for-all} model, where all cuts must be preserved simultaneously. We improve the previous $\Omega(n \sqrt{\beta/\epsilon})$ lower bound to $\tilde{\Omega}(n \sqrt{\beta}/\epsilon)$ in the for-each model, and we improve the previous $\Omega(n \beta/\epsilon)$ lower bound to $\Omega(n \beta/\epsilon^2)$ in the for-all model. This resolves the main open questions of (Cen et al., ICALP, 2021). The second problem is to approximate the global minimum cut in a local query model, where we can only access the graph via degree, edge, and adjacency queries. We improve the previous $\Omega\bigl(\frac{m}{k}\bigr)$ query complexity lower bound to $\Omega\bigl(\min\{m, \frac{m}{\epsilon^2 k}\}\bigr)$ for this problem, where $m$ is the number of edges, $k$ is the size of the minimum cut, and we seek a $(1+\epsilon)$-approximation. In addition, we show that existing upper bounds with slight modifications match our lower bound up to logarithmic factors.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> cut_query_ub.tex <==
\section{Discussion of Theorem~\ref{thm:cut_query_ub}}
\label{sec:appendix_query_ub}

We first give a high-level description of the algorithm in~\cite{globalmincut}. The algorithm is based on the following sub-routine.

\begin{lemma}
    There is an algorithm $\textsc{Verify-Guess}(D, t, \eps)$ which makes $\tilde{O}(\eps^{-2} m / t)$ queries in expectation and satisfies the following
    \begin{enumerate}
        \item If $t \ge \frac{2000 \log n}{\eps^2} \cdot k$, then $\textsc{Verify-Guess}(D, t, \eps)$ rejects $t$ with probability at least $1 - \frac{1}{\poly(n)}$. %,
        \item If $t \le  k$, then $\textsc{Verify-Guess}(D, t, \eps)$ accepts $t$ and output a $(1 \pm \eps)$-approximation of $k$ with probability at least $1 - \frac{1}{\poly(n)}$.
    \end{enumerate}
\end{lemma}

Given the above sub-routine, the algorithm initializes a guess $t = \frac{n}{2}$ for the value of the minimum cut $k$ and proceeds as follows:
\begin{itemize}
    \item if $\textsc{Verify-Guess}(D, t, \eps)$ rejects $t$, set $t = t / 2$ and repeat the process.
    \item if $\textsc{Verify-Guess}(D, t, \eps)$ accepts $t$, set $t = t/\kappa$ and let $\tilde{k} = \textsc{Verify-Guess}(D, t, \eps)$ and return the value of $\tilde{k}$ as the output, where $\kappa = \frac{2000\log n }{\eps^2}$ .
    
\end{itemize}

To analyze the query complexity of the algorithm, notice that when $\textsc{Verify-Guess}$ first accepts $t$, we have that 
%\[
$\frac{k}{2} < t < \kappa k$.
%\]
which means that $t/\kappa < k$ and hence one call to $\textsc{Verify-Guess}(D, t/\kappa, \eps)$ will get the desired output. However, at a time in $\Theta(t/\kappa)$, the $\textsc{Verify-Guess}$ procedure needs to make $\tilde{O}\big(\frac{m}{\eps^{4}k}\big)$ queries in expectation.

To avoid this, the crucial observation is that, during the above binary search process the error parameter of $\textsc{Verify-Guess}(D, t, \eps)$ is not needed to be set to $\eps$, but rather a small constant $\beta_0$ is sufficient. Then when $\textsc{Verify-Guess}(D, t, \beta_0)$ first accepts $t$, we have 
%\[
$\frac{k}{2} < t < c \log(n) \cdot k$,
%\]
where $c$ is a constant. Hence, the output of $\textsc{Verify-Guess}(D, t/(c \log n), \eps)$ will satisfy the error guarantee. Following the same analysis of that in~\cite{globalmincut}, we get that the query complexity of the new algorithm is $\tilde{O}(\frac{m}{\eps^{2}k})$.

==> cut_size.tex <==
\section{Figure of Lemma~\ref{lem:for_each_unit}}
\begin{figure}[h]
        \centering
        \includegraphics[width=0.8\linewidth]{figure.png}
        \caption{For $S = A \cup(R \setminus B)$,
    the edges from $S$ to $(V \setminus S)$: the forward edges are from $A$ to $B$, each with weight $O(\log(1/\eps))$; and the backward edges are from $(R \setminus B)$ to $(L \setminus A)$, each with weight $1/\beta$.}
        \label{fig:for_Each}
\end{figure}

% \begin{proof}
\section{Proof of Lemma~\ref{thm:k-connected}}
\label{app:proof}

To prove this, we use some properties about $\gamma$-connectivity of a graph. A graph is \textit{$\gamma$-connected} if at least $\gamma$ edges must be removed from $G$ to disconnect it. In other words, if a graph $G$ is $\gamma$-connected, then $\mathrm{MINCUT}(G) \geq \gamma$. Equivalently, a graph $G$ is $\gamma$-connected if for every $u, v \in V$, there are at least $\gamma$ edge-disjoint paths between $u$ and $v$. Therefore, given $\mathrm{INT}(x,y) = \gamma$, if we can show that $G_{x,y}$ is $2 \gamma$-connected and there exists one cut of size exactly $2\gamma$, then we can show $\mathrm{MINCUT}(G_{x,y}) \ge 2 \gamma$. 
By the construction of the graph, it is easy to see that $\mathrm{CUT}(A \cup A', B \cup B')$ has size $2 \gamma$, since each intersection of $x,y$ produces two crossing edges in between. Therefore, all we need to show here is that if $\sqrt{N} \geq 3 \cdot \gamma$, then $G_{x,y}$ is $2 \gamma$-connected.

Similar to \cite{eden2017lower}, we prove this by looking at each pair of $u,v \in V$. Our goal is to show that for every $u,v \in V$, there exists at least $2\gamma$ edge-disjoint paths from $u$ to $v$.
\setcounter{case}{0} % reset the case counter
\begin{case} 
    \label{case:case1}
    $u, v \in A$ (or symmetrically $u,v \in A', B, B'$).
    For each pair $u, v \in A$, we have that there are at least $\ell - \gamma$ distinct common neighbors in $A'$. This is because one intersection at $x_{ij}$ and $y_{ij}$ implies that the edge $(a_i, a_j')$ is not contained in $E$, and would remove at most one common neighbor in $A'$. Since $\ell = \sqrt{N} \geq 3 \gamma$, we have that there are at least $\ell - \gamma \geq 2 \gamma$ distinct common neighbors in $A'$, which we denote by $u^{A'}_{1}, u^{A'}_{2}, \dots, u^{A'}_{2\gamma}$. Therefore, each path $u \rightarrow u^{A'}_i \rightarrow v$ is edge-disjoint, and we have at least $2\gamma$ edge-disjoint paths from $u$ to $v$, as shown in \Cref{fig:case1}.
    \begin{figure}[h]
        \centering
        \includegraphics[width=\linewidth]{img/graph_case1.jpeg}
        \caption{$u, v \in A$. We omit all the $(a_i, b_j')$, $(b_i, b_j')$, and $(b_i, a_j')$ edges.}
        \label{fig:case1}
    \end{figure}
\end{case}

\begin{case}
\label{case:case2}
    $u \in A, v \in A'$ (or symmetrically $u \in B, v \in B' $).
    Since $\ell - \gamma \geq 2 \gamma$, we have that $v$ has at least $2\gamma$ distinct neighbors in $A$, which we denote by $u^{A}_1, u^{A}_2, \dots, u^{A}_{2\gamma}$. From Case~\ref{case:case1}, we also have that each $u^{A}_i$ has at least $2 \gamma$ distinct common neighbors in $A'$. Therefore, we can choose $v^{A'}_1, v^{A'}_2, \dots, v^{A'}_{2\gamma}$ such that each path $u \rightarrow v^{A'}_i \rightarrow u^{A}_i \rightarrow v$ is edge-disjoint, so we have at least $2\gamma$ edge-disjoint paths from $u$ to $v$, as shown in \Cref{fig:case2}. Note that it may be the case where $u^{A}_i = u$. In this case, we can simply take the edge $(u, v)$ to be one of the edge-disjoint paths.

    \begin{figure}[h]
        \centering
        \includegraphics[width=\linewidth]{img/graph_case2.jpeg}
        \caption{$u \in A, v \in A'$. We omit all the $(a_i, b_j')$, $(b_i, b_j')$, and $(b_i, a_j')$ edges. The green edges exist since $v$ has at least $2\gamma$ neighbors in $A$. The orange edges exist since $u^{A}_i$ and $u$ have at least $2\gamma$ common neighbors in $A'$. }
        \label{fig:case2}
    \end{figure}
\end{case}

\begin{case}
    \label{case:case3}
    $u \in A, v \in B'$ (or symmetrically $u \in A', v \in B$). 
    In this case, we show two sets of edge-disjoint paths, where each set has at least $\gamma$ edge-disjoint paths from $u$ to $v$, and the two sets of paths do not overlap. Overall, we have at least $2 \gamma$ edge-disjoint paths.

    The first set of paths $S_1$ uses the edges between $A'$ and $B$. Let $(w_1, x_1), (w_2, x_2), \dots, (w_{\gamma}, x_{\gamma}) \in A' \times B$ be the edges between $A'$ and $B$. Each of these edges represents one intersection in $x$ and $y$. Therefore, there are exactly $\gamma$ of them. From Case~\ref{case:case2}, we have that for every $w_i$, there are $2\gamma$ edge-disjoint paths from $u$ to $w_i$. Hence, for every $w_i$, we can choose a path from $u$ to $w_i$ and these $\gamma$ paths are edge-disjoint.
    \Cref{fig:case3.1} illustrates the paths $u \rightarrow u_i \rightarrow u'_i \rightarrow w_i \rightarrow x_i$. By symmetry, we can extend the paths from $x_i$ to $v$. This gives us $\gamma$ edge-disjoint paths from $u$ to $v$.

    \begin{figure}[h]
        \centering
        \includegraphics[width=\linewidth]{img/graph_case3.1.jpeg}
        \caption{$u \in A, v \in B'$. The first set of paths $S_1$ goes from $u \rightarrow u_i \rightarrow u'_i \rightarrow w_i \rightarrow x_i$. We omit the paths from $x_i$ to $v$, as they are symmetric to the paths from $w_i$ to $u$. Once we extend the paths from $x_i$ to $v$, we have $\gamma$ edge-disjoint paths from $u$ to $v$. Note that the $w_i$ and $x_i$ may not be distinct.}
        \label{fig:case3.1}
    \end{figure}

    We now consider the second set of paths $S_2$. Let $$(y_1, z_1), (y_2, z_2), \dots, (y_{\gamma}, z_{\gamma}) \in A \times B'$$ be the distinct edges between $A$ and $B'$. Once again, it suffices to prove that there are $2\gamma$ edge-disjoint paths from $u$ to $y_i$, since the paths between $v$ to $z_i$ would be symmetric. From Case~\ref{case:case1}, we have that for every $y_i$, there are at least $2\gamma$ common neighbors between $y_i$ and $u$. Therefore, we can always find distinct $u''_1, u''_2, \dots, u''_{\gamma}$ such that the paths $u \rightarrow u''_i \rightarrow y_i$ are edge-disjoint, as shown in \Cref{fig:case3.2}. Once we extend the paths from $z_i$ to $v$, we have $\gamma$-edge disjoint paths in the second set.

    \begin{figure}[h]
        \centering
        \includegraphics[width=\linewidth]{img/graph_case3.2.jpeg}
        \caption{$u \in A, v \in B'$. The second set of paths $S_2$ goes from $u \rightarrow u''_i \rightarrow y_i \rightarrow z_i$. We omit the paths from $z_i$ to $v$, as they are symmetric to the paths from $y_i$ to $u$. Once we extend the paths from $x_i$ to $v$, we have $\gamma$ edge-disjoint paths from $u$ to $v$. Note that the $y_i$ and $z_i$ may not be distinct.}
        \label{fig:case3.2}
    \end{figure}

    Now we have two sets of paths $S_1$ and $S_2$, where both sets have at least $\gamma$ edge-disjoint paths. It remains to show that the paths in $S_1$ and $S_2$ can be edge-disjoint. Observe that the only possible edge overlaps between the paths from $u$ to the $w_i$ and paths from $u$ to the $y_i$ are $u \rightarrow u''_i$ and $u \rightarrow u_i$, since they are both neighbors of $u$. However, note that what we have shown is that for every $w_i$ or $y_i$, there are at least $2\gamma$ edge-disjoint paths from $u$ to $w_i$ or $y_i$. Therefore, one can choose $2\gamma$ edge-disjoint paths from $u$ to $w_i$ and $y_i$ such that $u_i'$ and $u_i''$ do not overlap. And similarly one can choose $2\gamma$ edge-disjoint paths from $v$ to the $z_i$ and the $x_i$. Overall, we have $2 \gamma$ edge-disjoint paths from $u$ to $v$.
\end{case}
    
\begin{case}
    $u \in A, v \in B$ (or symmetrically $u \in A', v \in B'$).
    This case is similar to Case~\ref{case:case3}, where we have two edge-disjoint sets $S'_1$ and $S'_2$. Consider the set of paths $S'_1$, where we use the edges $$(w_1, x_1), (w_2, x_2), \dots, (w_{\gamma}, x_{\gamma}) \in A' \times B.$$ We can construct the paths from $u$ to $w_i$ using the same way as for $S_1$ in Case~\ref{case:case3} (\Cref{fig:case3.1}). For the paths from $x_i$ to $v$, however, we construct them using the same way as in $S_2$ in Case~\ref{case:case3} (\Cref{fig:case3.2}). By connecting these paths, we obtain at least $\gamma$ edge-disjoint paths in $S'_1$. Similarly, we can also construct at least $\gamma$ edge-disjoint paths in $S'_2$, where we use the edges $$(y_1, z_1), (y_2, z_2), \dots, (y_{\gamma}, z_{\gamma}) \in A \times B'.$$ We follow the same way of choosing the paths in $S'_1$ and $S'_2$ that are edge-disjoint. \qedhere 
\end{case} 
% \end{proof}
